Type-safe, Polyvariadic Event Correlation

The pivotal role that event correlation technology plays in todays applications has lead to the emergence of different families of event correlation approaches with a multitude of specialized correlation semantics, including computation models that support the composition and extension of different semantics. However, type-safe embeddings of extensible and composable event patterns into statically-typed general-purpose programming languages have not been systematically explored so far. Event correlation technology has often adopted well-known and intuitive notations from database queries, for which approaches to type-safe embedding do exist. However, we argue in the paper that these approaches, which are essentially descendants of the work on monadic comprehensions, are not well-suited for event correlations and, thus, cannot without further ado be reused/re-purposed for embedding event patterns. To close this gap we propose PolyJoin, a novel approach to type-safe embedding for fully polyvariadic event patterns with polymorphic correlation semantics. Our approach is based on a tagless final encoding with uncurried higher-order abstract syntax (HOAS) representation of event patterns with n variables, for arbitrary $n \in \mathbb{N}$. Thus, our embedding is defined in terms of the host language without code generation and exploits the host language type system to model and type check the type system of the pattern language. Hence, by construction it impossible to define ill-typed patterns. We show that it is possible to have a purely library-level embedding of event patterns, in the familiar join query notation, which is not restricted to monads. PolyJoin is practical, type-safe and extensible. An implementation of it in pure multicore OCaml is readily usable.

==> effects-primer.tex <==
\subsection{A Primer on Effects and Handlers in Multicore OCaml}\label{polyjoins:sec:effects-handlers-ocaml}
\todo{try to make this section shorter} We embed \corrl{} into the multicore OCaml
dialect with native support for effects and handlers~\cite{dolan2017concurrent}. Here, we
give a short primer on how to program with effects and handlers in multicore OCaml.
%
Algebraic effects and handlers~\cite{Plotkin:2003aa,Plotkin:2009aa} enable structured programming
with user-defined effects in functional languages.
% Compared to more established language abstractions for effects, \ie,
% monads~\cite{Moggi:1991aa,Wadler:1992aa} and monad transformers~\cite{Liang:1995aa},
% effects and handlers compose more freely and conveniently, because they support modular
% instantiation and modular abstraction via effect interfaces~\cite{Kammar:2013aa}.
%
Intuitively, effects and handlers generalize
\lstinline[language=poorman]|try/catch/throw| for managed exceptions by enabling evaluation to resume
back to the point in the program, where the effect was ``thrown'', as a form of
coroutine~\cite{Moura:2009aa}.

Effects are invocations of named commands having a type signature.
%These distinctions are often conflated into just the term ``effect''.
For example, this declares
a failure effect:
\begin{lstlisting}[numbers=none]
effect Fail: unit -> 'a
\end{lstlisting}
It consists of the command \lstinline|Fail|, taking a unit-valued argument and returning any
type. Its polymorphic return type indicates that it cannot resume to the calling site, because
failures are not supposed to return.
%
Effect commands are invoked with \lstinline|perform|, \eg,
\begin{lstlisting}
let be_positive () =
  let i = read_int () in (* Read positive integer from keyboard *)
  if i > 0 then i else perform (Fail ())
\end{lstlisting}
In multicore OCaml, effects can be handled by the existing language facilities for exception
handling, in cases of \lstinline|try| blocks. By handling command invocations,
we give them an implementation/semantics. A handler may map failure to proper exceptions:
\begin{lstlisting}[numbers=none]
try be_positive () with
| effect (Fail ()) k -> failwith "work on your attitude!"
\end{lstlisting}
or alternatively, may provide a default positive number:
\begin{lstlisting}[numbers=none]
try be_positive () with
| effect (Fail ()) k -> 42
\end{lstlisting}
Just as exceptions, command invocations are dynamically dispatched to the innermost handler
in the evaluation context having a matching clause. That is, effect handling is a form
of dynamic overloading.
However, effect handlers also bind the resumption of the underyling computation, which
can be invoked via \lstinline|continue|, e.g.,
given the command
\begin{lstlisting}[numbers=none]
effect Read: unit -> int
\end{lstlisting}
the expression
\begin{lstlisting}
try (perform (Read ())) + 1 with
| effect (Read ()) k -> continue k 41
\end{lstlisting}
evaluates to \lstinline|42|.

% \todo{MM: really relevant for the discussion in this paper?}
% While commands have type signatures. Multicore OCaml does not track \emph{effect
% types} in function arrows, as other languages do. For example, it infers the type \lstinline|be_positive: unit -> int|,
% which does not expose that \lstinline|Fail| may occur. Consequently, it is currently not possible to
% statically ensure that all effects are handled in multicore OCaml.

%As in the work by Bra\v{c}evac et al.,
We use functions to lift second-class \lstinline|try|
handlers into first-class effect handlers, \eg,
\begin{lstlisting}
let handler: (unit -> 'a) -> 'a = fun action ->
  try action () with
  | effect (Fail ()) k -> 42
\end{lstlisting}
And define a binary composition \lstinline@|+|@ on first-class handlers:
\begin{lstlisting}[numbers=none]
let (|+|) h1 h2 action = h1 (fun () -> h2 action)
\end{lstlisting}
which nests handlers in right (innermost) to left (outermost) order.

% \paragraph*{Generative Effects}%
% What are generative effects?

% \subsubsection{Event Patterns from Effects}\label{polyjoins:sec:event-patterns-from}

% In this paper, we investigate a restriction of Definition~\ref{polyjoins:def:joins}, which is relevant for
% query languages: we fix dimension (\ref{polyjoins:itm:constructors}) to a single type constructor\seba{I was
%   wondering why it's interesting to vary the C anyways. Can we explain that?}, but let the other
% dimensions vary freely:
% $$R[A_1]\times \cdots \times R[A_n] \Rightarrow R[A_1\times\cdots\times A_n].$$
% We can achieve type-safe polyvariadic definitions for such joins in OCaml, without ad-hoc
% polymorphism or dependent types, using more modest type system features: GADTs and modules.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "report"
%%% End:


==> fig-cartesius-var.tex <==
\begin{figure}
  \centering
\begin{lstlisting}[aboveskip=0pt,belowskip=-5pt]
module \corrl{}Vars = struct
  (* Variables carry generative effect instances *)
  type _ var =  Bind: ('a shape repr * 'a slot) -> 'a repr var (*@\label{polyjoins:lst:cartesius-var-var}@*)
  (* Generative effect creation *)
  let mk_slot: type a. a shape repr -> a slot = (*@\label{polyjoins:lst:cartesius-var-mkslot}@*)
    (module struct
       type t = a (* Type-level linking of input and effect *)
       < cf. Figure (*@\ref{polyjoins:fig:slotsignature}@*) >
     end: (SLOT with type t = a))
  module Ctx = HList(struct type 'a t = 'a var end)
  type 'a ctx = 'a Ctx.hlist
  (* from bindings change accordingly *)
  let from shape = Bind (shape, mk_slot shape) (*@\label{polyjoins:lst:cartesius-var-from}@*)
  let cnil = Ctx.nil
  let (@.) = Ctx.cons
end
\end{lstlisting}
  \caption{\corrl{} Variable Representation.}\label{polyjoins:fig:cartesius-var}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "report"
%%% End:


==> fig-fireexampleocaml.tex <==
\begin{figure}[t]
  \centering
\begin{lstlisting}[belowskip=-10pt,aboveskip=0pt]
join ((from temp_sensor) @. (from smoke_sensor) @. cnil) (*@\label{polyjoins:lst:taglessfireexample:context}@*)
       (fun ((temp,t1), ((smoke,t2), ())) -> (*@\label{polyjoins:lst:taglessfireexample:binders}@*)
          where (within t1 t2 (minutes 5.0)) %& smoke %& (temp %>= 50.0)
            (yield (format "Fire %f" temp))) (*@\label{polyjoins:lst:taglessfireexample:body_end}@*)
\end{lstlisting}
\caption{Polyvariadic Fire Example Event Pattern in \polyjoin{}/OCaml.}\label{polyjoins:fig:fireexampleocaml}
\end{figure}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "report"
%%% End:


==> fig-hlistfunctions.tex <==
\begin{figure}[h]
  \centering
\begin{lstlisting}
module HMAP(S:hlist)(T:Hl) = struct
  type ftor = {f: 'a. 'a S.el -> 'a T.el}
  let rec map: type a. ftor -> a S.hlist -> a T.hlist =
    fun {f} -> function
    | S.Z -> T.Z
    | S.S (h,t) -> T.S (f h, map {f} t)
end
\end{lstlisting}
\begin{lstlisting}
module HFOREACH(H:Hl) = struct
  type foreach = {f: 'a. 'a H.el -> unit}
  let foreach: type a. foreach -> a H.hlist -> unit =
    fun {f} hs ->
      let module U =
        HList(struct type 'a t = unit end) in
      let module M = HMAP(H)(U) in
      ignore @@ M.map {M.f = f} hs
end
\end{lstlisting}
\caption{Generic Heterogeneous List Functions.}\label{polyjoins:fig:hlistfunctions}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "report"
%%% End:


==> fig-injection.tex <==
\begin{figure}\centering
\begin{lstlisting}[aboveskip=0pt,belowskip=-5pt]
module type InjectSymantics = sig
  type 'a repr
  type ('ctx,'a) shape
  type 'ctx ext
  val empty_ext: unit -> 'ctx ext
  val (|++|): 'ctx ext -> 'ctx ext -> 'ctx ext
  val inject: 'ctx ext -> ('ctx,'a) shape repr  -> (unit,'a) shape repr
  val yield: 'a repr -> ('ctx, 'a) shape repr
  val join: 'a ctx -> ('a -> ('c,'b) shape repr) -> ('c,'b) shape repr
end
\end{lstlisting}
 \caption{Tagless Final Signature for Dependency Injection}\label{polyjoins:fig:inject-symantics}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "report"
%%% End:


==> fig-memory-handler.tex <==
\begin{figure}
  \centering
\begin{lstlisting}[aboveskip=0pt,belowskip=-5pt]
let slot_list: (module SLOT) list = abstract slots (* Forget concrete types *)
let memory = gen_handlers slot_list (fun (s: (module SLOT)) ->
  let module S = (val s) in
  let mem: S.t list ref = ref [] in
    (fun action ->
       try action () with
         | effect (S.GetMail) k -> continue k !mem
         | effect (S.SetMail l) k -> mem := l; continue k ()))
\end{lstlisting}
  \caption{Example: Bulk Instantiation of Generative Effect Handlers.}\label{polyjoins:fig:memory-handler}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "report"
%%% End:


==> fig-signals-ex.tex <==
%\begin{figure}[h]
\begin{lstlisting}[aboveskip=0pt]
(* Combine latest join semantics. *)
let join_impl: type a. unit -> 'a Ctx.hlist -> ('a -> 'b signal) -> 'b signal =
  fun () ctx pattern ->
    let out_signal = fresh_signal () in
    let join_state = mk_state ctx in
    let callback () =
      extract () join_state (fun tuple ->
      let next_signal = pattern tuple in
      out_signal.push (next_signal.pull ()))
    in
    subscribe_all ctx callback;
    out_signal
\end{lstlisting}
\begin{lstlisting}[aboveskip=0pt]
(* Dynamic references. *)
type 'a dref = unit -> 'a
module JoinState = HList(struct type 'a t = 'a dref end)
let mk_state: type a. a Ctx.hlist -> a JoinState.hlist = fun ctx ->
  let module M = HMAP(Ctx)(JoinState) in
  M.map {M.f = fun (Bind s) -> s.pull} ctx
\end{lstlisting}
\begin{lstlisting}[aboveskip=0pt]
(* Bulk access of dynamic references. *)
let extract: type a b. unit -> a JoinState.hlist -> (a -> b) -> b =
  fun () state k ->
    let module M = HMAP(JoinState)(HL) in
    let values = M.map {M.f = fun dref -> dref ()} state
    in k (HL.to_tuple values) (* Projects an 'a HL.hlist to a tuple 'a *)
\end{lstlisting}
\begin{lstlisting}[aboveskip=0pt]
(* Bulk subscription to signals *)
let subscribe_all: type a. a Ctx.hlist -> (unit -> unit) -> unit =
  fun ctx callback ->
  let module F = HFOREACH(Ctx) in
  F.foreach {F.f = fun (Bind s) -> s.subscribe (callback)} ctx
\end{lstlisting}
 % \caption{Type-safe, Polyvariadic Implementation of Combine Latest Semantics.}\label{polyjoins:fig:ex-signals}
%\end{figure}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "report"
%%% End:


==> fig-zip-n.tex <==
\begin{figure}[t]
  \centering
\begin{lstlisting}[mathescape=true,belowskip=0pt,aboveskip=0pt]
(* To zip 0 lists, do nothing and return *)
let z k = k (*@\label{polyjoins:lst:zip-numerals:zero}@*)
(* To zip n+1 lists: *)
let s n k = n (fun zs_n -> (* first zip n lists into zs_n *)(*@\label{polyjoins:lst:zip-numerals:succ:start}@*)
                  (fun xs -> (* and given the (n+1)th list *)
                     k (zip_bin zs_n xs))) (* yield their binary zip *)                   (*@\label{polyjoins:lst:zip-numerals:succ:end}@*)
(* Index numbers embody the zip implementation, where
   the nth number yields an (n+1)-way zip: *)
let zip n = n (fun x -> x)(*@\label{polyjoins:lst:zip-numerals:zip}@*)
(* zip1: 'a list -> 'a list *)
let zip1 () = zip z(*@\label{polyjoins:lst:zip-numerals:examples:start}@*)
(* zip2: 'a list -> 'b list -> ('a * 'b) list *)
let zip2 () = zip (s z)
(* zip3: 'a list -> 'b list -> 'c list -> (('a * 'b) * 'c) list *)
let zip3 () = zip (s (s z))
(* example usage: *)
let xs = zip3 () [1] ["2";"3"] [4.0;5.0] (* yields [((1,"2"),4.0)] *)(*@\label{polyjoins:lst:zip-numerals:examples:end}@*)
\end{lstlisting}
  \caption{ML/OCaml $\phi$-number encoding of $n$-way \lstinline|zip| in continuation-passing style.}
  \label{polyjoins:fig:zip-numerals}
\end{figure}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "report"
%%% End:


==> ingredients.tex <==
\subsection{Event Patterns from Algebraic Effects}\label{polyjoins:sec:backgr-effectf-progr}

Our language defines declarative event patterns, reminiscent of standard language integrated query
(LINQ)~\cite{Meijer:2006aa,Cheney:2013aa} syntax, respectively monadic do/for notation.  In contrast
to these works, \corrl{} translates into a representation on top of algebraic effects and handlers
\cite{Plotkin:2003aa,Bauer:2015aa}, a recently proposed abstraction for specifying user-defined
effects that composes more conveniently than monads.

There is good reason to keep the monadic query style: convenient, familiar to end users.  However,
we argued that standard translations, which rely on nesting, are not adequate for event correlation,
because nesting introduces unnecessary control dependencies.  Instead, we argue for a translation
that favors parallel composition of bound expressions, instead of nesting.  Gap between the two:
syntax and binding structure is different from the structure of the generated computation, which
``untangles'' the nesting.

There are two notable aspects to \corrl{}: the need for safely supporting arbitrary arities, which
is a natural requirement for joining an arbitrary, but finite number of event sources and the heavy
use of generative effects. The latter are effects that need to be allocated dynamically, per event
correlation instance (prime example of generative effect: mutable references).  Generative effects
to date are not well-understood within the theory of algebraic effects, much less supported by state
of the art language implementations of this abstraction.

\subsubsection{Algebraic Effects and Handlers}%
\label{polyjoins:sec:algebr-effects-handl}

Primer on effects and handlers.

\paragraph{Generative Effects}%
\label{polyjoins:sec:generative-effects}

What are generative effects?

\subsubsection{The \corrl{} Language}%
\label{polyjoins:sec:mini-cartesius}

A (hopefully) small and lean version of our system.


\subsubsection{Joins in \corrl{}}
\label{polyjoins:sec:joins-cartesius}

In this paper, we investigate a restriction of Definition~\ref{polyjoins:def:joins}, which is relevant
for query languages: we fix dimension (\ref{polyjoins:itm:constructors}) to a single type constructor\seba{I was wondering why it's interesting to vary the C anyways. Can we explain that?},
but let the other dimensions vary freely:
$$R[A_1]\times \cdots \times R[A_n] \Rightarrow R[A_1\times\cdots\times A_n].$$
We can achieve type-safe polyvariadic definitions for such joins in OCaml, without ad-hoc
polymorphism or dependent types, using more modest type system features: GADTs and modules.


%\todo{add examples of concrete libraries/languages}

% \todo{is this really answer type polymorphism?}
% such as monadic versions, which is essentially a
% curried version of above signature, using bind... and answer-type polymorphism.
% joins can be specified using the standard monadic combinators
%   $\mathbf{return}\cln\; A \to \Type{M}[A]$ and $\mathbf{bind}\cln\; \Type{M}[A]\to (A\to\Type{M}[B])\to\Type{M}[B]$.
% For example,
% \begin{align*}
%   & \mathbf{let}\;\mathit{cartesian}_n = \lambda m_1\cln \Type{M}[A_1] \ldots \lambda m_n\cln \Type{M}[A_n].\\
%   & \quad\mathbf{bind}\; m_1\; (\lambda x_1\cln A_1.  \\
%   & \quad\qquad \mathbf{bind}\; m_2\; (\lambda x_2\cln A_2. \\[-2ex]
%   & \phantom{\quad\qquad \mathbf{bind}\; m_2\; (\lambda x_2}\ddots \\[-1ex]
%   & \qquad\qquad\qquad \mathbf{bind}\; m_n\; (\lambda x_n\cln A_n. \mathbf{return}\; \anglep{x_1,\ldots, x_n}) \ldots ))
% \end{align*}


$$\begin{tikzcd}[column sep=huge,row sep=huge]
  R[A_1]\times \cdots \times R[A_n] \arrow[r, "\varrho"] \arrow[d]
  & R[A_1\times\cdots\times A_n]  \\
  \thunk{\Type{Unit}}^{\anglep{\eff{push}_1,\ldots, \eff{push}_n,\varrho}} \arrow[r, "\anglep{\eff{yield},\eff{fail},\varrho}"] & \Type{Unit} \arrow[u, "\varrho"]
\end{tikzcd}$$




\section{Polyvariadic Definitions and Effects in Multicore OCaml}
\label{polyjoins:sec:techniques}

\todo{this is like a second background section, do we really need it? Should it be rather interleaved with 4?}

In this section, we recapitulate basic OCaml programming techniques, which we utilize in
\Cref{polyjoins:sec:case-study:-cart} for larger-scale polyvariadic programming.

\input{polyvariadic_intro}


% \subsection{Type Representation and Type Relations}
% \label{polyjoins:sec:type-repr-type}

% The constrained polymorphism of GADTs enables expressing complex relations at the type
% level. However, they induce a footprint at the level of values, \ie, to express type-level
% relations, we must construct term values that witness the type relation. Especially in our setting,
% we require creating and manipulating lists of types, which we define in the following.

% First of all, we require a type for witnessing OCaml types:
% \begin{lstlisting}
% type 'a typ = Typ
% let witness: 'a -> 'a typ = (fun _ -> Typ)
% \end{lstlisting}
% The type \lstinline|typ| has only one constructor \lstinline|Typ|, but has a phantom
% type~\cite{Leijen:1999aa} parameter to statically represent an arbitrary type.
% In order to obtain a type representation from a given value, the function \lstinline|witness|
% can be invoked with the value. Alternatively, explicit ascriptions can be used, \eg,
% \begin{lstlisting}[numbers=none]
% let typ_int: int typ = Typ
% \end{lstlisting}

% We represent lists of types by a heterogeneous list type similar to \lstinline|hlist| in
% \Cref{polyjoins:sec:abstr-over-heter}:
% \begin{lstlisting}
% type _ typ_list =
%   | TNil: unit typ_list
%   | TCons: ('a typ * 'b typ_list) -> ('a * 'b) typ_list
% \end{lstlisting}
% The difference is that each \lstinline|TCons| cell holds a type representation instead
% of an OCaml value.

% Now we can express type-level relations among lists of types with further GADTs.
% One important instance is a functional relation, where a list of types is
% related to the element-wise application of a type constructor.
% We express this relation by an OCaml module signature and
% functor, abstracting over the concrete type constructor:
% \begin{lstlisting}
% module type ElementWise = sig
%   type 'a wrap
%   type (_,_) proof =
%     | Base: (unit, unit) proof
%     | Step: ('a typ * 'a wrap typ * ('b, 'c) proof) ->
%                (('a * 'b), ('a wrap * 'c)) proof
%   ...
% end
% module ElementWiseWrap(T: sig type 'a wrap end):
%   (ElementWise with type 'a wrap = 'a T.wrap) = ...
% \end{lstlisting}
% The GADT \lstinline|proof| establishes a binary relation between its type arguments. We can think of
% the GADT constructor signatures as defining type-level inference rules and GADT values as concrete
% derivation trees, which can be inspected by pattern matching.  A concrete value of type
% \lstinline|(a,b)$\ $proof|
% describes a derivation of the fact that \lstinline|a| and \lstinline|b| are in the relation. In this
% instance, a value of type \lstinline|(a,b)$\ $proof|
% certifies that (1) both types \lstinline|a| and \lstinline|b| have the shape of nested tuples
% (hlist) of the same length $n$
% and (2) at each position $i\in \Set{0\ldots n-1}$
% in the tuple, we have that \lstinline|b$_i$ = a$_i$ wrap| for the supplied type constructor \lstinline|'a wrap|.

% There are two straightforward rules (constructors) for deriving the judgment
% \lstinline|(a,b)$\ $proof|.
% The first is the axiom \lstinline|Base|, specifying that trivially, the empty type lists are
% related. The second rule \lstinline|Step| inductively extends a proof that relates two type lists of
% length $n$
% to a proof relating extended type lists of length $n+1$.
% For this, the $(n+1)$th
% elements must be type witnesses, where the right witness stems from the left witness by applying the
% type constructor \lstinline|wrap|.

% Below is an example usage of type relations, which instantiates an \lstinline|ElementWise|
% relation with the standard \lstinline|list| type constructor.
% \begin{lstlisting}
% module ListWrap = ElementWiseWrap(struct type 'a wrap = 'a list end)
% open ListWrap
% let rec extract_hds: type a b. (a,b) proof -> b hlist -> a option =
%   fun proof hs ->
%     match proof, hs with
%       | Base, HNil -> Some ()
%       | Step (_,_,prev), HCons ([], tl) -> None
%       | Step (_,_,prev), HCons (x :: xs, tl) ->
%            bind (extract_hds prev tl) (fun tl -> Some (x,tl))
% \end{lstlisting}
% Using the \lstinline|proof| type of the relation, we specify the signature of the
% function \lstinline|extract_hds|. Given an arbitrary hlist of lists, it extracts
% the hlist containing all the heads of the input lists, if each of them is non-empty.
% This is an example usage:
% \begin{lstlisting}
% let hlist1 = HCons ([1], HCons (["2"], HCons ([3.0], HNil)))
% let hlist2 = HCons ([1], HCons ([], HCons ([3.0], HNil)))
% let proof = Step (int_typ, (list_typ int_typ),
%                    Step (string_typ, (list_typ string_typ),
%                       Step (float_typ, (list_typ float_typ), Base)))
% let v1 = extract_hds proof hlist1  (* Some (1, ("2", (3.0, ()))) *)
% let v2 = extract_hds proof hlist2  (* None *)
% \end{lstlisting}
% In later sections, we will address how to avoid letting end-users write \lstinline|proof| values by
% hand.

% \subsection{$\phi$-number Signatures}
% \label{polyjoins:sec:phi-numb-sig}

% Let us revisit zip and look at the types of z and s.

% Capture signature as variadic gadt


% \begin{lstlisting}
% module Zip = struct
%   module Sig = struct

%   end
% end
% \end{lstlisting}
% Synthesis from signature: standard and staged.

% \subsection{Context-dependent Variadic Definitions}
% \label{polyjoins:sec:cont-depend-vari}

% We do bottom up construction (folding), how to deal with context-dependence. Think accumulator-style
% definitions. Prime example: Reversal of hlists.

% \subsection{Composing Polyvariadic Definitions}
% \label{polyjoins:sec:comp-polyv-defin}

% Holed expressions vs. signatures.

% Incremental construction.

% Need to stay in open form...

% Programming holed expressions and signatures...
% Holes in GADTs

% \subsection{Strongly-typed, Variadic Modules}
% \label{polyjoins:sec:strongly-typed-modules}

% Signature: module with proof objects
% Instance: functor on signature

% \begin{lstlisting}
% module ListWrap = ElementWiseWrap(struct type 'a wrap = 'a list end)
% module type Constrained = sig
%   type x
%   type y
%   val p_y_wraps_x: (x,y) ListWrap.proof
% end
% \end{lstlisting}

% Sometimes it is acceptable to use abstract
% representation. (think forall handler).


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "report"
%%% End:


==> polyvariadic_intro.tex <==
\subsection{Polyvariadic Programming with $\phi$-Numbers}\label{polyjoins:sec:polyvariadic_programming}

\todo{it seems the role of the numerals greatly decreased now, this section will likely go}

Polyvariadic programming
refers to type-safe encodings of abstractions having a variable number of parameters, which are
heterogeneously typed. One example is a generalization of the standard \lstinline|zip| combinator,
which combines two lists into a list of pairs, to a version combining $n$
lists to a list of $n$-tuples,
for arbitrary $n \geq 1$.  Informally, its type signature (in OCaml notation) should have the shape
\begin{lstlisting}[mathescape=true,numbers=none,xleftmargin=.1\textwidth]
zip$_n$: 'a$_1$ list -> $\cdots$ -> 'a$_n$ list -> ('a$_1$ * $\cdots$ * 'a$_n$) list$,\ n\geq 1.$
\end{lstlisting}
That is to say, we would like to define a number-indexed \emph{family} of \lstinline|zip| functions
in a typed implementation language.

Remarkably, it is possible to define polyvariadic combinators using nothing more than the basic
Hindley-Milner (HM) type system. Of such approaches, we study the ad-hoc number encoding by
Fridlender and Indrika~\cite{Fridlender:2000aa}, which we call \emph{$\phi$-numbers} for brevity\seba{why do we study those? are we using or extending them?}.

\input{fig-zip-n}

To illustrate $\phi$-numbers
in action, we define an ML/OCaml implementation of \lstinline[mathescape=true]|zip$_n$|
in \Cref{polyjoins:fig:zip-numerals}. Lines~\ref{polyjoins:lst:zip-numerals:zero}-\ref{polyjoins:lst:zip-numerals:succ:end} define
the combinators \lstinline|z| (zero) and \lstinline|s| (successor) for constructing the
$\phi$-numbers
of \lstinline|zip$_n$|\seba{what does that mean? are we constructing numbers or functions?}.
Together they constitute an inductive definition over the index number $n$
for a continuation-passing style (CPS) implementation of \lstinline[mathescape=true]|zip$_n$|:
The base step at number $0$
is trivial, and the inductive step at number $n+1$
extends the implementation at $n$ with the standard binary zip function, which we call \lstinline|zip_bin|.

Lines~\ref{polyjoins:lst:zip-numerals:zip}-\ref{polyjoins:lst:zip-numerals:examples:end} of \Cref{polyjoins:fig:zip-numerals}
demonstrate how to instantiate \lstinline|zip$_n$| in client code,
for concrete index numbers $n$.
Note that each instance has the correct type.\footnote{There are some immaterial
  differences from the previous informal signature: the \lstinline|zip$_n$| functions construct nested
  pairs, instead of proper $n$-tuples
  and indexing is zero-based, \ie, \lstinline|zip| at number $n$
  combines $n+1$
  lists. } The point is that polyvariadic definitions from $\phi$-numbers
are simple and convenient to use in client code, since they directly and immediately express the
concept of number-indexing: to obtain the $n$-th
element of the family, simply pass the $n$-th
$\phi$-number constructed from \lstinline|z| and \lstinline|s|.
\seba{the example is great but needs more explanation to make sure everybody understands the definition of z and s.}

\seba{What was the point of showing the zip example? What have we learnt? How does this help/influence our solution?}

% For example, higher-kinded polymorphism and ad-hoc overloading with
% implicits/type classes~\todo{[???] strictly speaking, ml functors enable hk-poly too} or dependent
% types~\cite{Weirich:2010ab,Weirich:2010aa} have been used in the context of polyvariadic programming
% already. However, to the best of our knowledge, little is known so far outside of
% folklore about the combination of $\phi$-numbers
% with (1) generalized algebraic data types (GADTs)~\cite{Johann:2008aa} and (2) first-class
% modules~\todo{[???]}, which are two distinguished features of modern OCaml.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "report"
%%% End:

